Processing and Segmentation of Human Teeth from 2D Images using Weakly Supervised Learning

Teeth segmentation is an essential task in dental image analysis for accurate diagnosis and treatment planning. While supervised deep learning methods can be utilized for teeth segmentation, they often require extensive manual annotation of segmentation masks, which is time-consuming and costly. In this research, we propose a weakly supervised approach for teeth segmentation that reduces the need for manual annotation. Our method utilizes the output heatmaps and intermediate feature maps from a keypoint detection network to guide the segmentation process. We introduce the TriDental dataset, consisting of 3000 oral cavity images annotated with teeth keypoints, to train a teeth keypoint detection network. We combine feature maps from different layers of the keypoint detection network, enabling accurate teeth segmentation without explicit segmentation annotations. The detected keypoints are also used for further refinement of the segmentation masks. Experimental results on the TriDental dataset demonstrate the superiority of our approach in terms of accuracy and robustness compared to state-of-the-art segmentation methods. Our method offers a cost-effective and efficient solution for teeth segmentation in real-world dental applications, eliminating the need for extensive manual annotation efforts.

==> figures/annotation-tool.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.5\textwidth]{pictures/annotation-tool.png}
    \caption{The annotation tool interface. Left: Image that the doctor can click on. Right: Annotation tags.}
    \label{fig:annotation-tool}
\end{figure}

==> figures/automatic-thresholding.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[\centering Original image.]{{\includegraphics[width=0.32\textwidth]{diploma-thesis/pictures/a-thresh-orig.png} }\label{a-thresh-orig}}%
    \quad
    \subfloat[\centering Grayscale variant of \protect\subref{a-thresh-orig}.]{{\includegraphics[width=0.285\textwidth]{diploma-thesis/pictures/a-thresh-gray.png} }\label{a-thresh-gray}}%
    \quad
    \subfloat[\centering Otsu's thresholding of \protect\subref{a-thresh-gray}.]{{\includegraphics[width=0.285\textwidth]{diploma-thesis/pictures/a-thresh.png} }\label{a-thresh}}%
    
    \subfloat[\centering Morph. closing of \protect\subref{a-thresh}.]{{\includegraphics[width=0.34\textwidth]{diploma-thesis/pictures/a-thresh-close.png} }\label{a-thresh-close}}%
    \quad
    \subfloat[\centering Hole filling of \protect\subref{a-thresh-close}.]{{\includegraphics[width=0.285\textwidth]{diploma-thesis/pictures/a-thresh-fill.png} }\label{a-thresh-fill}}%
    \quad
    \subfloat[\centering Applied mask.]{{\includegraphics[width=0.29\textwidth]{diploma-thesis/pictures/a-thresh-mask.png} }\label{a-thresh-mask}}%
    \caption{Example of automatic thresholding for lower jaw.}
    \label{fig:a-thresh}%
\end{figure}

==> figures/centernet.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{diploma-thesis/pictures/objects-as-points.png}
    \caption{Example of bounding box definition from \cite{Centernet}. Here, the bounding box is defined as center point (x, y) and a width and height.}
    \label{fig:objects-as-points}
\end{figure}

==> figures/feature-maps.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{pictures/feature-maps.png}
    \caption{Convolutional filters applied on a an image of teeth. Each picture is an application of one filter. Filter activations are brighter and non-activated regions are dark.}
    \label{fig:feature-maps}
\end{figure*}

==> figures/feature-model.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{pictures/feature-model.drawio-4.png}
    \caption{Derivation of our proposed feature model from ResNet18 architecture. It makes use of several feature maps from ResNet18 by combining them together with 1x1 convolution operations.}
    \label{fig:feature-model}
\end{figure}

==> figures/front-view-problem.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.35\textwidth]{diploma-thesis/pictures/problem-hm-front.png}
    \caption{Predicted heatmap for an image of front view.}
    \label{fig:problem-hm-front}
\end{figure}

==> figures/heatmaps.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[\centering 2D heatmap of Gaussian kernels. Zero values are black, higher values are bright.]{{\includegraphics[width=0.35\textwidth]{diploma-thesis/pictures/heatmap.png} }\label{2d}}%
    \quad
    \subfloat[\centering 3D view of the heatmap in \protect\subref{2d}.]{{\includegraphics[width=0.35\textwidth]{diploma-thesis/pictures/hm_3d.png} }\label{3d}}%
    \quad
    \caption{Example of heatmap for lower jaw. \protect\subref{2d} 2D heatmap. \protect\subref{3d} 3D view.}
    \label{fig:heatmaps}%
\end{figure}

==> figures/histogram.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Image of lower jaw in grayscale.]{{\includegraphics[width=0.35\textwidth]{diploma-thesis/pictures/gray.png} }\label{gray}}%
    \quad
    \subfloat[\centering Histogram of \protect\subref{gray}.]{{\includegraphics[width=0.5\textwidth]{diploma-thesis/pictures/histogram.png} }\label{hist}}%
    \quad
    \caption{Example of grayscale image processing. \protect\subref{gray} Grayscale image. \protect\subref{hist} Histogram.}
    \label{fig:heatmaps}%
\end{figure}

==> figures/hsv-thresholding-results.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Prediction mask.]{{\includegraphics[width=0.4\textwidth]{diploma-thesis/pictures/hsv-thresh-pred.png} }\label{hsv-pred}}%
    \quad
    \subfloat[\centering Ground-truth mask.]{{\includegraphics[width=0.4\textwidth]{diploma-thesis/pictures/hsv-thresh-gt.png} }\label{hsv-gt}}%
    \caption{Example of semantic segmentation using HSV thresholding.}
    \label{fig:hsv-thresholding-results}%
\end{figure}

==> figures/hsv.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Image converted to HSV color space visualized using RGB color space.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/hsv-image.png} }\label{hsv-a}}%
    \quad
    \subfloat[\centering HSV color space histogram of \protect\subref{hsv-a}.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/hsv-histogram.png} }\label{hsv-hist}}%
    \quad
    \subfloat[\centering Mask selecting light blue color.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/mask-a.png} }\label{mask-a}}%
     \quad
    \subfloat[\centering Mask selecting everything except blue colors.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/mask-b.png} }\label{mask-b}}%
     \quad
    \subfloat[\centering Logical OR using \protect\subref{mask-a} and \protect\subref{mask-b}.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/mask-c.png} }\label{mask-c}}%
     \quad
    \subfloat[\centering Morphological hole filling applied on \protect\subref{mask-c}.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/mask-d.png} }\label{mask-d}}%
    \caption{Example of exploiting the HSV color space of an image. 
    \protect\subref{hsv-a} HSV spectrum of original image.
    \protect\subref{hsv-hist} HSV histogram.
    \protect\subref{mask-a} Mask selecting light blue color.
    \protect\subref{mask-b} Mask selecting everything except blue colors.
    \protect\subref{mask-c} Logical OR using \protect\subref{mask-a} and \protect\subref{mask-b}.
    \protect\subref{mask-d} Morphological hole filling applied on \protect\subref{mask-c}.}
    \label{fig:analytical-results}%
\end{figure}

==> figures/inpainted.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Original image]{{\includegraphics[width=0.44\textwidth]{diploma-thesis/pictures/not-inpainted.png} }\label{not-inpainted}}%
    \quad
    \subfloat[\centering Inpainted image.]{{\includegraphics[width=0.44\textwidth]{diploma-thesis/pictures/inpainted.png} }\label{inpainted}}%
    \caption{Example of inpainting algorithm.}
    \label{fig:inpainted}%
\end{figure}

==> figures/irnet.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=1.1\textwidth]{diploma-thesis/pictures/irnet-model.png}
    \caption{The complete pipeline from \cite{IRNet}. In the bottom-left corner we can see the Inter-pixel Relation Network, whose two outputs are displacement field and class boundary map. These outputs are combined with the class activation maps later in the process.}
    \label{fig:irnet-model}
\end{figure}

==> figures/keypoint-results.tex <==
\begin{figure*}[t!]
    \centering
    \subfloat[\centering Prediction on front view.]{{\includegraphics[width=0.3\textwidth]{pictures/hourglass-results-front-a.png} }\label{hourglass-front-a}}%
    \quad
    % \subfloat[\centering Prediction on front view.]{{\includegraphics[width=0.35\textwidth]{pictures/hourglass-results-front-b.png} }\label{hourglass-front-b}}%
    % \subfloat[\centering Prediction on lower jaw.]{{\includegraphics[width=0.35\textwidth]{pictures/hourglass-results-bottom.png} }\label{hourglass-bottom}}%
    % \quad
    \subfloat[\centering Prediction on upper jaw.]{{\includegraphics[width=0.3\textwidth]{pictures/hourglass-results-top.png} }\label{hourglass-top}}%
    \caption{Example of keypoint prediction with CenterNet (Hourglass backbone). Dark purple markers represent ground-truth keypoints, turquoise markers represent predictions.}
    \label{fig:keypoint-results}%
\end{figure*}

% \protect\subref{hourglass-front-a} and \protect\subref{hourglass-front-b} are examples of front view.

==> figures/maskrcnn.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=\textwidth]{diploma-thesis/pictures/maskrcnn.png}
    \caption{Results of Mask R-CNN model on COCO dataset.}
    \label{fig:maskrcnn}
\end{figure}

==> figures/our-method-pipeline.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Feature map.]{{\includegraphics[width=0.24\textwidth]{diploma-thesis/pictures/feature-map.png} }\label{our-fm}}%
    \quad
    \subfloat[\centering Thresholded.]{{\includegraphics[width=0.21\textwidth]{diploma-thesis/pictures/thresholded.png} }\label{our-thresh}}%
    \quad
    \subfloat[\centering Morph. closed.]{{\includegraphics[width=0.21\textwidth]{diploma-thesis/pictures/closed.png} }\label{our-closed}}%
    \quad
    \subfloat[\centering Refined with CRF.]{{\includegraphics[width=0.21\textwidth]{diploma-thesis/pictures/refined.png} }\label{our-crf}}%
    
    \subfloat[\centering Watershed distances.]{{\includegraphics[width=0.24\textwidth]{diploma-thesis/pictures/watershed-distances.png} }\label{our-distances}}%
    \quad
    \subfloat[\centering Predicted keypoints area.]{{\includegraphics[width=0.21\textwidth]{diploma-thesis/pictures/keypoints-area.png} }\label{our-keypoints-area}}%
    \quad
    \subfloat[\centering Distances with keypoints area.]{{\includegraphics[width=0.21\textwidth]{diploma-thesis/pictures/distances-with-area.png} }\label{our-distances-keypoints-area}}%
    \quad
    \subfloat[\centering Final mask.]{{\includegraphics[width=0.21\textwidth]{diploma-thesis/pictures/final-mask.png} }\label{our-final-mask}}%
    \caption{Processing pipeline of our method.}
    \label{fig:our-method-pipeline}%
\end{figure}

==> figures/our-results.tex <==
\begin{figure*}[htbp]
    \centering
    \subfloat[\centering Prediction on lower jaw.]{{\includegraphics[width=0.2\textwidth]{pictures/our-result-bot.png} }\label{our-result-bot}}%
    \quad
    \subfloat[\centering Prediction on front view.]{{\includegraphics[width=0.2\textwidth]{pictures/our-result-front.png} }\label{our-result-front}}%
    \quad
    \subfloat[\centering Prediction on upper jaw.]{{\includegraphics[width=0.2\textwidth]{pictures/our-result-top.png} }\label{our-result-top}}%
    
    \subfloat[\centering Ground-truth mask of lower jaw.]{{\includegraphics[width=0.2\textwidth]{pictures/gt-bot.png} }\label{gt-bot}}%
    \quad
    \subfloat[\centering Ground-truth mask of front view.]{{\includegraphics[width=0.2\textwidth]{pictures/gt-front.png} }\label{gt-front}}%
    \quad
    \subfloat[\centering Ground-truth mask of upper jaw.]{{\includegraphics[width=0.2\textwidth]{pictures/gt-top.png} }\label{gt-top}}%
    \caption{Example of results from our proposed solution.}
    \label{fig:our-results}%
\end{figure*}

==> figures/problem-prediction.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[\centering Heatmap generated by CenterNet model.]{{\includegraphics[width=0.35\textwidth]{diploma-thesis/pictures/problem-hm.png} }\label{problem-hm}}%
    \quad
    \subfloat[\centering Predicted keypoints from heatmap.]{{\includegraphics[width=0.35\textwidth]{diploma-thesis/pictures/problem-prediction.png} }\label{problem-prediction}}%
    \quad
    \caption{Example of wrong keypoint prediction for lower jaw.}
    \label{fig:problem-prediction}%
\end{figure}

==> figures/resnet-all-graphs.tex <==
\begin{figure*}[t!]
    \centering
    \subfloat[\centering Results from model with output size 128x128 pixels.]{{\includegraphics[width=0.47\textwidth]{pictures/resnet18_all_128_0.png} }\label{resnet-all-128}}%
    \quad
    \subfloat[\centering Results from model with output size 512x512 pixels.]{{\includegraphics[width=0.47\textwidth]{pictures/resnet18_all_512_0.png} }\label{resnet-all-512}}%
    \caption{Precision, recall and f1 score for different distance threshold values. \protect\subref{resnet-all-128} Model with smalle output size. \protect\subref{resnet-all-512} Model with larger output size.}
    \label{fig:resnet-all-0}%
\end{figure*}

==> figures/sam-prediction-top.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Predicted mask from SAM on image of upper jaw.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/sam-pred-top.png} }\label{sam-pred-top}}%
    \quad
    \subfloat[\centering Ground-truth mask.]{{\includegraphics[width=0.3\textwidth]{diploma-thesis/pictures/sam-gt-top.png} }\label{sam-gt-top}}%
    \caption{Example of SAM prediction on image.}
    \label{fig:sam-prediction-top}%
\end{figure}

==> figures/sam.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=\textwidth]{diploma-thesis/pictures/sam.png}
    \caption{Architecture of Segment Anything Model from \cite{SAM}.}
    \label{fig:sam-model}
\end{figure}

==> figures/sequence-example.tex <==
\begin{figure}[b!]
    \centering
    \subfloat[\centering Image of upper jaw.]{{\includegraphics[width=0.47\textwidth]{diploma-thesis/pictures/top.png} }\label{upper}}%
    \quad
    \subfloat[\centering Image of lower jaw.]{{\includegraphics[width=0.47\textwidth]{diploma-thesis/pictures/bottom.png} }\label{lower}}%
    \quad
    \subfloat[\centering Image of front view.]{{\includegraphics[width=0.6\textwidth]{diploma-thesis/pictures/front.png} }\label{front}}%
    \caption{Example of one patient's sequence. \protect\subref{upper} Upper jaw. \protect\subref{lower} Lower jaw. \protect\subref{front} Front view.}
    \label{fig:sequence-example}%
\end{figure}

==> figures/true-positives.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{pictures/true-positives.png}
    \caption{Example case of classification false positives and false negatives. Blue markers represent ground-truth keypoints, green markers represent predictions.}
    \label{fig:true-positives}
\end{figure}

==> figures/whats-the-point-results.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{diploma-thesis/pictures/what-the-point-results.png}
    \caption{Qualitative results of their model on the PASCAL VOC 2012 validation set. The model trained with image-level labels usually predicts the correct classes and their general locations,
but it over-extends the segmentations. The objectness prior improves the accuracy of
the image-level model by helping infer the object extent. Point supervision aids in
separating distinct objects (row 2) and classes (row 4) and helps correctly localize the
objects (rows 3 and 4). Best viewed in color.}
    \label{fig:whats-the-point-results}
\end{figure}

==> howto.tex <==
\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\input{tables/keypoint-results-all-images}

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

==> sections/approach.tex <==
\section{Approach}
In this section we will describe the overall approach or overview of the solutions we are proposing regarding different tasks.
\subsection{The Annotation Tool}
% \input{figures/annotation-tool}
\input{figures/feature-maps}
It is commonly known that there is a significant lack of medical data in general, but when it comes to annotated medical data, the deficit is even bigger. Therefore, we decided to develop a tool that could help dentists to easily annotate images of human teeth. Thus, we were greatly motivated, because if annotated medical data can be produced easily and made accessible, it would bring more options and opportunities to machine learning and data science fields to progress and bring benefits to medicine and other fields. Our task seemed quite simple at first: develop a tool for dental image annotation that could be easily shared, accessed and used by every dentist. We decided to develop it as a web application with a simple NoSQL database and host it on Google Firebase.

The application was mainly designed to make the process of annotating images as comfortable and fast as possible. Each patient is associated with image sequences (sequences for short). Patients can have multiple image sequences and each sequence can be annotated only once. These sequences consist of three images each, while the three images correspond to the lower jaw, upper jaw and the last one is a frontal view of the teeth. To tell sequences apart from one another, each sequence is defined as the date and time the images were taken on.

The doctor can open up a sequence of any patient and start the annotation process. First image in the sequence is automatically loaded and displayed for the dentist. The mouse acts as a pointer to the center of each tooth, so the dentist is supposed to click inside a tooth to mark its center point. The relative coordinates of the center are saved and the annotation form appears. He or she can then fill the properties that applies to the selected tooth. By repeating this process for each tooth on the image, and for each image in the sequence, we end up with whole sequence annotated, which is three images worth of information in total. After that, the doctor is prompted to fill in some information, which applies globally to the whole sequence (overall health of the patient's teeth etc.). The doctor can then review his annotation by looking at a table that contains all the filled information about each tooth. After this review process the doctor can submit the annotation and the data is uploaded to a server, from which we can download the stored data and process it further. 

\subsection{Keypoint prediction}
\input{tables/keypoint-results-basic}

For this part of our work we have all the labels we need, therefore we can leverage fully supervised training for creating our model. However, results of this part will have a strong influence on the segmentation task, because it is going to be essentially an extension of this task.

The prediction of keypoints is a problem, in which for an image of human teeth our goal is to get a list of coordinates, each corresponding to the center point of one tooth. The keypoint prediction problem is not at all a new kind of problem, since almost every object detection algorithm is solving this task in some way. Conveniently, convolutional neural network models (such as object detectors or pose estimators) were also created and train to tackle these kinds of problems, and they have proven to yield satisfying results \cite{Centernet}. As we mentioned earlier, we are going to adopt a CenterNet architecture \cite{Centernet} and train it for on our dataset. The core idea behind this architecture is viewing objects as single points in an image with corresponding width and height values rather than two key points (upper left and lower right corners) \cite{yolo}. This is very fortunate for us, because our annotations encode each tooth as a single point. That is why the choice of this architecture was very natural. Since the CenterNet model is able to predict width and height of an object additionally to the key point, we can simplify it by removing the corresponding output branches, leaving out only the branch for key point output.

We will be using a CenterNet architecture with ResNet \cite{resnet} backbone, which is a good and overall simple feature extraction model. CenterNet takes a 2D image as an input and outputs a 2D heatmap of Gaussians, which peaks correspond to the locations of key points of object instances. This is a convenient solution, because it easily overcomes the problem of varying number of object predictions, which is a common obstacle when modeling an object detector. Generally, one heatmap for one object class is created, but in our case there will always be only a single heatmap. 

As an evaluation metric, we compute the euclidian distance in pixels between the ground truth keypoints and predicted ones. Note that we do not have the information about which keypoint belongs to which tooth in particular, meaning the ground truth keypoints are unordered. Because of this, we cannot directly compute the error regarding a specifig tooth, e.g. the first molar. This problem can be solved by pairing predicted keypoint with ground truth keypoints using the Hungarian algorithm \cite{hungarian}. Then we can take the paired keypoints from this algorithm and compute the distance between them in pixels. These values can be then averaged to get the mean distance error and also the distance median.
\input{figures/resnet-all-graphs}

\subsection{Semantic segmentation}
The proposed solution for this task will be dependent to a large extent on the keypoint prediction solution. Semantic segmentation can be viewed as classification of individual pixels into classes semantically. In the context of our problem, we will have only 2 classes, teeth and gum. For this task we do not have any annotations at all, so fully supervised learning is not possible in this case. That is why our focus will be mainly on weakly supervision. This type of supervision tries to obtain the maximum potential out of features learned by some model. These learned features are contained in the weights (filters) of the trained model and usually can be visualized by applying the learned convolutional filters on an input image. Since each filter in each convolutional layer is trying to detect different features, we get different results by applying different filters. We can see an example of such visualization in Fig. \ref{fig:feature-maps}, where we applied filters from one of the first convolutional layers of our network. Inspired by Feature Pyramid networks \cite{fpn} and IRNet architectures \cite{IRNet}, we combine together feature maps from multiple layers in the model and get a rich feature representation of teeth in the image. The reason why this is useful for us is because if we can obtain such an image, where the teeth are represented differently that everything else on that image, that is a great starting point for segmentation algorithms. In fact, we will process such image further with some analytical algorithms and then also try to use the predicted points as well.

Apart from our own proposed approach, we will also be implementing some analytical solutions for image segmentation as well as some new state-of-the-art deep learning solutions \cite{cutler}, \cite{SAM} to see, how well each one one these methods perform. Going from the simplest methods to the most advanced, we will start with algorithms such as automatic thresholding of grayscale images and thresholding using HSV masks, then proceed to implement feature extraction model from our trained keypoint prediction model and at last we will have a look at the two new transformer architectures mentioned above.
% \subsubsection*{Automatic thresholding}
% This method is very simple one, which utilizes the grayscale histogram of the image. First, an image is converted into grayscale color space and histogram of the number of white pixels per certain threshold is created. Then the algorithm finds the threshold value, which is the most optimal one and all values below this threshold are turned to black and values above are turned to white. 
% \subsubsection*{HSV thresholding}
% Another type of thresholding algorithm is thresholding based on the hue, saturation and value. This works by manually selecting range of values for a mask. If we select a particular range that would correspond to the red color for example, we can then select every pixel that falls into this range of colors and segment it from everything. We will implement this type of thresholding with two masks, each having its own range of colors for selection.
% \subsubsection*{Pre-trained MaskCut and DINO models}
% Inspired by \cite{cutler}, we can use pretrained self-supervised transformer architecture DINO \cite{DINO} and pass its learned features to MaskCut \cite{cutler} to perform self-supervised segmentation. It is a new paradigm of using vision transformers, because it is essentially a zero-shot detector that was trained self-supervised. We will only use its pre-trained weights for semantic segmentation.
% \subsubsection*{Segment Anything Model}
% We will also try the new pre-trained Segment Anything Model \cite{SAM}. It works in two main modes: automatic and with point supervision. In the automatic mode, the model is only prompted with an image and outputs one or more segmentation masks. In the mode with point supervision, we can prompt the model with reference points in an input image, and the model will try to segment only that part of the image, which the point refers to. This can be very conveniently combined with our model for keypoint prediction, because then we can prompt the model with points referring to individual teeth, improving the segmentation masks.


==> sections/conclusion.tex <==
\section{Conclusion}  % chapter* je necislovana kapitola
In this work we have focused on the processing of dental images. The images we used in this thesis mainly come from a publicly available dataset \cite{Invisalign}, which contains images of three different types. Firstly, we have implemented web application that serves as a online annotation tool for dentists, which specializes on annotating images of human teeth.
% We believe that human annotations are a very valuable component in machine learning and that our tool can help minimize the lack of annotated medical data. During our initial collaboration with professional dentists we have hoped to recieve an annotated dataset of images of human teeth. But unfortunate events have forced us to annotate the images in our dataset ourselves using our own tool. Because of this, we were left with only simple annotations, which contained only the approximate coordinates of each tooth in an image. Having such annotations, the main goal of this work was to explore the field of weakly supervised learning and show how these simple annotation labels could potentially be used for semantic segmentation of teeth. We began by designing a deep learning model that was trained in the traditional fully supervised manner, which could predict the keypoints of each tooth in an input image. For the model, we used the popular CenterNet \cite{Centernet} architecture with ResNet18 \cite{resnet} backbone, and we made some minor modifications and adjustments to suit our needs. We have evaluated the model using mean and median distance error in pixels between the predicted and ground-truth keypoints. The model proved to be quite capable of solving this task, but showed some problems on certain type of input images. Therefore, we tried various data augmentation methods but they did not prove to provide better results. Additionally we tried implementing different, stronger backbones for the model, and they showed a raise in performance. The Stacked Hourglass backbone \cite{Centernet} proved to be best performing backbone.

The keypoint prediction model served as a foundation for our weakly supervised pipeline for semantic segmentation. After the fully supervised training of the model, we examined the learned features by this model and by manually picking out certain convolutional layers, we constructed a new model. This new model is capable of predicting such feature maps from input images, that the most activated regions represented the locations of teeth. Hence, these feature maps were very convenient for further processing. We have applied multiple analytical algorithms on top of these feature maps and we have even made use of the predicted keypoints themselves. As a result, we have ended up with a model capable of semantic segmentation of human teeth. For evaluation purposes, we decided to implement four additional methods for semantic segmentation. Two of those methods are completely analytical, meaning they do not use any type of machine learning algorithm or training processes, and two of them are state-of-the-art unsupervised deep learning models based on the vision transformer architecture.  The results in Table \ref{table:summary-results} show that our model is the best performing one. Our proposed method even outperformed the new Segment Anything Model \cite{SAM} when prompted with keypoints. This shows that using only keypoints as additional guide does not suffice in obtaining the best results. We showed that the feature maps predicted by our proposed model are the key component in our weakly supervised pipeline in Table \ref{table:thresholding-comparison}.

During our work, we have discovered new approaches and methods that can be studied in order to bring more improvements into this type of problem. Vision transformer architectures and self-supervised learning paradigms are becoming more popular tools in the field of semantic segmentation of images. Nonetheless, we consider the major contribution of this work to be the validation of weakly supervised pipeline, which we believe can add value to this field of research.

==> sections/introduction.tex <==
\section{Introduction}
The majority of neural networks models (classifiers and detectors) are trained fully supervised, meaning that during training for each input the model is provided corresponding label or ground truth. This way, the training process is very efficient and often result in good performance of the network because we have a full supervision over the training of the model. In other words, we provide the network with exactly what we want the network to learn. However for this to achieve, a great amount of data is needed. The more data we have, the better performance our model is likely to have. And this is one of the main problems of machine learning even to this day - data insufficiency.

Proper annotated and ground truth data can only be made by humans, manually. Surely, for simple tasks such as image classification, only image level labels are required, which can be made quite tirelessly today (through global approaches like image captcha etc.). But more complex tasks require more complex annotations, e.g. instance segmentation, which requires each pixel painted manually. The insufficiency of annotated data for instance segmentation tasks gets even greater when it comes to medical data. Because with medical data, two problems arise. One being the protection of privacy information. Due to this problem, majority of the medical datasets cannot be published online. Some of them are only intended usually for some closed local research of a small group of scientists. Second problem is that annotations themselves are needed to be done by a certain doctor or specialist. This reduces the number of people eligible to make these annotations to a very small number. Thus large public annotated medical datasets almost do not even exist. Therefore, in recent years, researchers in deep learning were also focusing on how to overcome this problem of data shortage. And surprisingly, new interesting approaches were presented. Probably the most exciting ones are called semi-supervised learning and weakly supervised learning. Both are concerning the training process and are meant to replace the traditional full supervision. In semi-supervised training, some of data are annotated and some are not (without any labels). In weakly supervised training, all of data is annotated, but not completely. Weak supervision requires more complicated pipeline than full supervision, because it treats the data differently. In general, we do not provide the network with exactly what we want as an output. But instead, we provide it with so called weak labels. These weak labels can be of many different types. Besides already mentioned image level labels, centers of objects (points) or even squiggly lines inside the objects were tested and proven to work.

Our work was highly motivated to explore the field of weak supervision in order to overcome the problem of insufficient amount of annotated data. We have worked with medical data, specifically with dental images and we have tried different experiments and various methods, that can be used to process images with deep learning. Our primary goal was to train such neural network that can perform keypoint prediction and see if this predictions can help us towards semantic segmentation of rgb images of human teeth. These images came mainly from two sources. First one being public unannotated dataset [to be edited] and second one being small group of dentists that we were in contact during first stages of this thesis. This problem also has a practical background or rather, its solution has a practical use. Imagine having a tool (maybe an app in your mobile phone) that could automatically perform basic dental anamnesis or even detect various tooth diseases. To develop such complex and advance tool, the ability to detect and segment teeth from gums is the first major step towards this goal. Therefore, the aim of this work is threefold: 
\begin{itemize}
    \item implement custom web annotation tool for dentists,
    \item train a deep learning model for teeth keypoint prediction of each tooth in an image,
    \item show that such model together with weak labels (keypoints) can be used and expanded to perform semantic segmentation of teeth in an image.
\end{itemize}

==> sections/related-work.tex <==
\section{Related Work}

\subsection{Objects as points}
Authors of this work \cite{Centernet} proposed a model of convolutional neural network for object detection based only on one keypoint - center of the object. Other popular detectors \cite{MaskRCNN} iterate through a large number of possible object locations multiple times, classifying each one if it contains an object or not. This process is very resource exhausting and requires additional post-processing, and often causes a significant performance bottleneck. CenterNet \cite{Centernet}, model name proposed by authors, estimates only the center points of objects, and then proceeds to predict the width and height of objects. It can have ResNet \cite{resnet} module or Stacked Hourglass module \cite{Centernet} as backbones. At the end of the network, there are three output heads: first to predict center key points, second to predict width and height and third to predict offset values for the keypoints. The first head which estimates key points produces a heatmap (one for each class, generally of size 128x128 pixels) of Gaussian peaks, which represent the locations of center points. The second and third output heads produce a regression values at those peak locations for width, height and offset. Another important property of this model is that it does not require the traditional IoU (intersection over union) based non-maximum suppresion to filter out wrong key point predictions. It was proven in the article that using it in the post-processing stage results in only a minor impact, therefore they do not use it. CenterNet is famous for its simple principles and architecture and at the same time for providing promising results. In our work, we adopt this architecture and tweak it to our needs. We will go in more implementation details in future chapters.

\subsection{Segment Anything Project}
Worldwide known company Meta recently released a project called Segment Anything \cite{SAM}, which caused a major breakthrough in computer vision and deep learning. The whole project comprises of many different components, but the three major ones are task, model and dataset for image segmentation. These components are to be the foundation of a promptable model for image segmentation. With such model, the authors aim to solve a wide range of segmentation tasks using prompt engineering. The task component is essentially a promptable segmentation task proposed by authors, inspired by foundation models in natural language processing and computer vision, which goal is to produce a valid segmentation mask given any prompt. The prompt should specify what part of the image should segmented and by valid segmentation mask they mean a reasonable mask even when the prompt is ambiguous, e.g. if the prompt is a single point on a person wearing a t-shirt, valid output would be mask for either the person or the t-shirt. For the second component, the model, this imposes great constraints and expectations together with real-time inference for interactive use. However, the authors come up with a simple design that satisfies these constraints: a prompt encoder for encoding segmentation prompts, an image encoder for computing image embeddings, and a lightweight mask decoder which combines the previous two to decode segmentation masks. These three parts form the Segment Anything Model (SAM). The separation of the model into image encoder and prompt encoder is a key principle, because this way one image can be used with different prompts while preserving the same image embedding and therefore saving computational time. The problem of prompt ambiguity is solved by returning multiple masks for a single prompt, e.g. mask for a t-shirt as well as mask for a person in the problem mentioned before. Motivated by scalability and powerful pre-training methods they use visual transformers as the image encoder, altered to process high resolution images. On the output end, the mask decoder is also built from transformer architecture. It is a modified transformer decoder block with a mask prediction head. The last component in the whole project is the data engine with the dataset. Segment Anything Data Engine is used to create a large-scale dataset for image segmentation. It can be used in three different modes (assisted-manual, semi-automatic, and fully automatic) and can also run in the browser. The dataset created (SA-1B) now consists of around one billion annotated images, which are publicly accessible. The results of this work are really impressive, as they now compete some of the state-of-the-art fully supervised object detectors.
\subsection{Point-level Supervision}
In this article \cite{ThePoint}, the authors have introduced a point-level supervision for semantic segmentation for the first time to their knowledge. The authors were aware of fully supervised state-of-the-art CNN models used for semantic segmentation, but they were trying to take weakly supervised methods a step further. They knew that detailed per-pixel annotations were very time consuming and therefore searched for another approach, that would not need such costly labels but still have comparable results. At that time, only image-level class labels, bounding boxes, squiggly lines and few others were being used as the weak labels. The authors are saying they "took a natural step" from image-level supervision to point-level supervision. Meaning their approach uses a bit stronger supervision that image-level labels, but the annotation time is fairly similar. According to the authors, for a human to refer to an object, the most natural way is to point to it. The annotators were asked to just point to an object on an image. The annotated data had one point inside each object class. Then they incorporated the point supervision to a loss function in an existing state-of-the-art model.
% An issue that they faced is that models with very few pixels supervised have a problem inferring the right spatial extent of an object. This means that the models can learn the relative position of the objects in an image, but have a tendency to make the segmentation mask bigger than the actual objects. In other words, they are prone to a local minima. To overcome this problem, they used a objectness priors. Objectness priors provide a probability for whether each pixel belongs to any object class as opposed to background. It is essentially something that we know \textit{prior} to the actual segmentation process. These priors are gathered from a pre-trained objectness detectors. Having point-level annotations and objectness priors, they trained a state-of-the-art fully convolutional network with a VGG16 \cite{vgg} backbone having its layers converted to convolutional ones. At the end they replaced the classifier layer with 1x1 convolution layer with number of filters equal to the number of classes.
\subsection{Instance segmentation using peak class response}
Extending and enabling classification network for instance segmentation, this was the motivation of authors of this work \cite{peak-response}. They were motivated by the fact that classification networks trained with image-level labels can produce class response maps (or class activation maps), which correspond to the classification confidence of different image regions. Moreover, that local maxima, or peaks, of these regions often resemble highly contributing parts of different instances of objects in the image. To obtain these peaks, they first converted the classifier network into a fully convolutional network, which preserve spatial information and produce a class response maps in a forward pass. Then they constructed a peak stimulation layer that is inserted after the top layer. The input to this layer is a class response map and the output is a class-wise confidence scores, meaning that each peak is associated with a class score. Because the class response maps are usually of a small size and low resolution, they are alone insufficient for segmentation. That is why the authors propose to further backpropagate the stimulated class-wise confidence scores (peaks) to generate a more informative regions of each object, referred to as peak response maps. The backpropagation of peaks is a probabilistic process, and the authors say we can imagine it as if a random walker starts walking randomly from the top layer all the way to the bottom. Then a top-down relevance of each object is formulated at the bottom layer as the object probability of being visited by the random walker. With this probability propagation the most relevant spatial locations of each object can be localized and used to create the peak response maps.  These maps are fine-detailed and can be further exploited for instance segmentation of objects. They have implemented this with ResNet50 \cite{resnet} and VGG16 \cite{vgg} architectures and evaluated in multiple benchmark datasets. It seems so that they were the first ones to perform instance segmentation using pre-trained classifier network.

==> sections/results.tex <==
\section{Results and Experiments}
In this section, we are going to show the results from both keypoint prediction and semantic segmentation and also look at what different kinds of experiments can be done to obtain different results. Firstly, we will take a look at how we evaluated and collected results from different solutions and what methods we used for evaluation. Then we will show some visualizations for better understanding.
\subsection{Keypoint prediction}
\input{figures/keypoint-results}
We implemented a CenterNet architecture to predict keypoints of each tooth in an image. At first, we did not make any changes to the dataset, so we trained CenterNet on the whole dataset with all images. This consists of 3 233 images of teeth, lower jaw, upper jaw and front view altogether, each one having resolution of 512x512 pixels. We can see the results from this training in Table \ref{table:keypoint-results-basic}. To our surprise, the mean error of the model with smaller output size shows better performance than the model with heatmap output size the same as input image. But as we already discussed, this could be caused by few images with significantly worse predictions, because if we look at the median values, they are almost the same in both cases.
\input{figures/our-results}

Additionally to the two metrics in Table \ref{table:keypoint-results-basic}, we also calculated a precision, recall and f1 score for each model. The motivation behind these three metrics is to include the fact that the model can sometimes predict different number of keypoints than the ground-truth contains. Because so far, the Hungarian algorithm leaves out the keypoints that do not have a pair. We think that the ability of the model to predict the right number of keypoints is crucial as well. For the three new metrics to be calculated, we need to count the number of true positives, false positives and false negatives. For that to be possible we use moving distance threshold. By using a certain threshold, we can divide our predicted keypoints into true positives and false positives by checking if \textbf{their distance from its paired keypoint is lower than the threshold}. If it is, we count the predicted keypoint as true positive (it is close enough to the ground-truth keypoint), if not, we count it as false positive. We collect the false negatives by counting the number of ground-truth keypoints that do not have a pair after using the threshold, because these are keypoints that should have been predicted, but our model did not predict any keypoints close enough. This way, if a model predicts different number of keypoints that there actually should be, they get classified as false positives and are included in our metric. Since choosing one fixed threshold would be insufficient for evaluating the full potential of the model, instead we calculate these metrics across a range of thresholds and depict it in a graph. We chose a range of 30 distance thresholds from 0 to 29. If we would have trained a model with no error at all, it would achieve the best scores for a distance threshold of 0. Since that is only a hypothetical scenario, our model gradually achieves better results as the distance threshold gets larger and larger, see Fig. \ref{fig:resnet-all-0}.
\input{tables/summary-results}

As an experiment, we wanted to see how would the model perform, if it was trained on specific subsets of our dataset. If we look at the images in our dataset, we see that the images of lower and upper jaw are quite similar in structure, they only differ in the curvature along which the teeth are located. The front view is quite different from the rest, firstly because the teeth are placed along a horizontal line, secondly there are almost twice as many teeth as in the other images and thirdly, there is a perspective distortion. By distortion we mean that the teeth are getting visually closer to each other as they approach the left and right border of the image. This causes the keypoints in the ground-truth heatmap to be very closely squeezed together. It becomes very hard for the model to predict the right locations of individual teeth in such cases. Another reason for splitting out dataset into subsets is an imbalance of images. As we know, we manually annotated $\sim$1000 image sequences, where there are two similar images (lower and upper jaw) and one is different (front view). We believe that this imbalance may have also caused model performance issues. Hence, we split our dataset into four subsets: images of lower jaw only, upper jaw only, front view only and images of lower and upper jaw only. The idea of the last subset arises from similarity in those two types of images mentioned earlier. We make sure to train four different models on these four different subsets of images exclusively and also to test the models on these subsets respectively. Table \ref{table:keypoint-results-basic} shows results of this experiment and we can clearly see that the front view is indeed very problematic. Now however, the model with output resolution of 512x512 pixels seemed to have performed better than the other one, as the median error for this model is lower in all cases and mean in three cases out of four. Particularly interesting are the results for the front view in the bottom row, as the difference between the mean and median error is significantly large. As in our first training, we think that it may have been caused by a few very poor predictions. Nonetheless, these results show noticable performance gains by training on separate dataset subsets.

% So far our model was implemented with the ResNet18 backbone, which is the simplest one. We were interested to see if stronger backbones could increase the model performance. Thus, we have implemented our model also with Resnet50 and Stacked Hourglass backbones. In Table \ref{table:keypoint-results-backbones} we show their results. We decided to leave out the lower jaw only and upper jaw only subsets of training images, because the model performance is similar for those two. Both of these models performed better with the larger output resolution than with the smaller one, and even results for all images is better than by the previous model with ResNet18 backbone. The mean error also dropped in all three training cases compared to the previous model. CenterNet with Stacked Hourglass module achieves the best results for the front view only dataset and also has really great and stable performance on the dataset with all images included. Training with stronger and more advanced backbones showed some performance gains, but they are also more resource demanding as we had to train the ResNet50 backbone only with batch size of 8 samples and the Hourglass backbone with batch size of 2 samples.
% \input{tables/keypoint-results-backbones}

In the Fig. \ref{fig:keypoint-results} we show the visualizations of keypoint prediction with the Stacked Hourglass backbone trained on all images. It is clear from the pictures \ref{hourglass-front-a} and \ref{hourglass-top} that predictions on front view images are a lot harder to make as the teeth can be positioned in various ways. On the other hand, predictions on lower jaw images and upper jaw images are a lot easier (hence the lower error values), since on such images there is no perspective distortion and the teeth are organized in a more predictable way.

\subsection{Segmentation}
\input{tables/feature-map-thresholding}

Now, we will show results from different methods for semantic segmentation. We want to make an important note here, that since we did not have mask annotations for our dataset, we manually created these masks ourselves for 30 images (10 images for each type of view, lower/upper jaw and front view). Meaning that all evaluations of semantic segmentation were made on this small subset of images. As evaluation metrics, we use traditional intersection over union (IoU), precision, recall and f1 score.
% Additionally, we tried removing reflections from our images in dataset with Navier-Stokes inpainting algorithm \cite{navier}. This algorithm inpaints the bright white spots in our images with the surrounding colors. We applied this algorithm to every image in our dataset and thus created a equally large second dataset. Motivation behind this decision was that we noticed the original images contained a lot of reflections, which often caused artifacts in segmentation masks. We wanted to see if such inpainting of reflections can help our segmentation methods.

% We will now go through each of our proposed methods of segmentation and show their performance on segmentation masks and tables with metrics. 
\textbf{Automatic thresholding.}
% \input{figures/automatic-thresholding}
% \input{tables/a-thresh-results}
The simplest method we have implemented for semantic segmentation is the automatic thresholding of grayscale images. 
% In Fig. \ref{fig:a-thresh} we can see the complete pipeline from this method. 
The original image gets converted to grayscale color space, then a rough binary mask is created using Otsu's thresholding \cite{otsu}. This rough masks is then further refined with morphological closing and hole filling algorithms to get rid of artifacts as much as possible. 
% Fig. \ref{a-thresh} shows an example application of this method only on bottom jaw, but we can see in Table \ref{table:a-thresh-results} that this method really struggles on the images of front view. 
Interestingly enough, there is noticable difference in performance between lower jaw only images and upper jaw only images. It is also evident that recall of this method increases with the inpainted dataset.

\textbf{HSV thresholding.}
% \input{tables/hsv-thresh-results}
% \input{figures/hsv-thresholding-results}
The second analytical method we have implemented is the thresholding using two masks for HSV color space.
% We have already explained the pipeline of this method in Fig. \ref{fig:analytical-results}. The first thing we can notice in the results from this method in Table \ref{table:hsv-thresh-results} is that 
It handles the images of front view far better than the previous method. 
% Also, there are almost no performance gains when tested on the inpainted images. Unlike in the previous method, where recall was better for the inpainted images, now the exact opposite is the case. In Fig. \ref{fig:hsv-thresholding-results} we can see an example mask prediction for an image of front view.

\textbf{Weak supervision using feature maps and keypoints}
% \input{tables/our-results}
% We have already illustrated the pipeline of our proposed method in Fig. \ref{fig:our-method-pipeline}. 
In the Table \ref{table:summary-results} we show results also from this method. There is a significant increase in performance compared to the previous methods in all three types of images. The model performed better with the original images for the lower jaw and front view datasets. We can see an example results from this method in Fig. \ref{fig:our-results}.

Since one of the key processes of our method is the initial thresholding of feature maps using Otsu's algorithm, which is the same for the first analytical method in this thesis, one can argue that our proposed method is only better because of the predicted keypoints. We consider the predicted feature maps from our model very valuable, as they contain important information about the location of teeth. To show their contribution to our pipeline, we decided to compare two types of binary masks: one produced by the automatic thresholding applied on original image, and the other one produced by same thresholding but applied on the predicted feature maps. In Table \ref{table:thresholding-comparison} we can see that the feature maps provide better building block for segmentation. The size of the dataset this was evaluated is not large enough as we mentioned earlier, but we still strongly believe that the results would still be better for the feature maps even for larger datasets.

\textbf{Pre-trained vision transformer and MaskCut}
From now we will focus on the models that use vision transformers. Starting with the first method, pre-trained DINO \cite{DINO} and MaskCut \cite{cutler} models. This approach is very interesting because it was not trained in the traditional fully supervised manner, but rather using self-supervision. However, we only adopted pre-trained weights, meaning that we did not perform any additional training. Looking at Table \ref{table:summary-results}, results from this method were not very promising. The model has the best results on the dataset with lower jaw only images, but even then the f1 score barely gets higher than 0.5. Since this model was not trained on our dataset at all, we were left with only setting the hyperparameters. Nonetheless, having considered that this model is not trained using ground-truth labels and still be able to produce rough masks of teeth is something worth noticing.
\input{tables/cutler-results}

\textbf{Segment Anything Model}
 \input{tables/sam-results}
% \input{figures/sam-prediction-top}
As our last solution we review the Segment Anything Model.  As we already mentioned, we tested this model both in automatic mode and in point supervision mode. In the automatic mode, SAM tries to detect every foreground object in the image. When using the point-supervised mode, we prompted SAM with keypoints from our keypoint prediction model, each marking one tooth as a foreground object. SAM in the automatic mode is obtaining similar results as previous method, CutLER. But using the predicted keypoints from our model and passing them to the model increases its performance by a significant amount. SAM is able to obtain noticeably better results in the point-supervised mode. 
% An example prediction of such image is illustrated in Fig. \ref{fig:sam-prediction-top}.

% \textbf{Summary}
% Now we will briefly summarize the results from all the methods used in this work and try to name few problems that came along the way as well as propose ideas for improvement and future work.

% Starting with the keypoint prediction model, we first saw interesting results, because higher output resolution did not seem to help achieve better results. But later we saw richer results by splitting the dataset into multiple subsets based on the image type. There we could see that the images of front view are very hard for predicting keypoints. We did try data augmentations of various types, but that did not prove to help achieve better results. At last we implemented the CenterNet model with stronger backbones, ResNet50 and Stacked Hourglass, and they showed noticeable gain in performance, especially the latter one. 

% For the segmentation problem we evaluated 5 different methods: automatic thresholding, thresholding of HSV color space, our proposed method, CutLER \cite{cutler} method and Segment Anything Model \cite{SAM}. Every segmentation method was evaluated on three subsets of our dataset separately to see, what if some images would be more problematic than other, as we have seen in the keypoint prediction problem. It is safe to say that the images of lower jaw only are the least uncertain, as each method achieved highest f1 score when evaluated on this subset of images. To our suprise, images of upper jaw only often caused lower values of f1 scores than images of front view only, even though we considered the lower jaw structurally very similar to the upper jaw. Major problems for the segmentation of front view images can be seen in the evaluation of our first method on the original dataset. However, when we tested the automatic thresholding on the inpainted dataset, a significantly better results were achieved on the front view images. But this was the only time the removal of reflections from our images helped to obtain results of higher quality. For every other method, the inpainted dataset showed very little or no improvement. 

% We decided to do a final evaluation of every method on the original dataset, without inpainted reflections and dataset subsets. By looking at the Table \ref{table:summary-results} we can see that our proposed method achieves the best results almost for every metric. Closest to ours, SAM prompted with keypoints achieves moderate results. From the two analytical methods, the thresholding of HSV color space seems to be the superior one.

% One important thing to measure when it comes to prediction is the inference time, or how long it takes for the model to predict a result. This can often be crucial, especially for real life applications, where models ought to be fast and precise. The fastest inference time has the simplest method, Otsu's thresholding combined with morphological operations, which can predict masks for 5 images under one second. The second analytical method, HSV thresholding, can predict 20 images under one second. This time difference might be due to the hole filling algorithm, which is used in the automatic thresholding and is very time consuming operation. The weakly supervised pipeline we proposed in this work is quite a complicated one, since it has to predict and use feature maps as well as the keypoints. This method predicts approximately one image per second. However, it is still faster then the Segment Anything model, which need around ten seconds to predict masks for one image using the automatic mode. But when prompted with keypoints, the inference time drops significantly and can then predict masks of one image per second. We measured the inference time of each method using the NVIDIA GeForce RTX 3060 graphics card. Unfortunately, these inference times are not at all suitable for video processing, as it requires inference of at least 20 images per second.

% \textbf{Problems and future work}
% \input{figures/problem-prediction}
% During the work on this thesis we have encountered a lot of obstacles. We managed to overcome some of them, but some are still an issue. There is essentially one major problem, which is tied to many others, and that problem lies within the keypoint heatmap prediction of CenterNet model. More precisely, the problem begins with inexact Gaussians in the heatmap. The Gaussians represent probabilities or confidence of locations where the teeth may be located, so when something on the image looks similar to a tooth, the model creates a small Gaussian on that location. 
% We can see an good example of this issue in Fig. \ref{fig:problem-prediction}, where in the image on the left we see a few smudged Gaussians circled in pink. These two peaks were high enough to made it through the maxpooling and thresholding operations and therefore they became keypoints in the final prediction. Sometimes the predicted heatmap contains more peaks than there are teeth (like in the previous example), and sometimes the heatmap contains less peaks than there are teeth in the image. This issue could be possibly solved by incorporating some heuristics, which would ensure that the predicted keypoints follow a certain curve along which the teeth are naturally placed. If we would have had the class label for each tooth (molar, premolar, incisor, etc.), this problem could be perhaps solved by training the model to classify each tooth to corresponding class.
% \input{figures/front-view-problem}

% Another problem that is closely related to the heatmap prediction is the problem with front view images, which became an reoccurring issue. If we look at such heatmap in Fig. \ref{fig:problem-hm-front}, on the left and right side of the heatmap the Gaussians are placed very closely to each other. They often get squeezed and smudged so much, that the keypoints extracted from such heatmaps contain a lot of error and usually the number of extracted keypoints does not match the ground-truth. But we do not consider this to be a problem of the model, rather than the image itself. The image of front view naturally has perspective deformation of teeth on the left and right side. The teeth appear very close to each other and thus it is very hard for the model to predict an accurate heatmap.

% As for segmentation problems, many of them arise from the wrong keypoint prediction. We have already explained how the keypoints help in the segmentation process, so it is obvious that incorrectly predicted keypoints cause a lot of segmentation problems. But there is one issue that remains the same even if the keypoints are predicted correctly. The issue is with amalgam fillings in the teeth and mainly concerns images of lower and upper jaw. Since these type of fillings have black color, if a keypoint falls inside this filling, the model often only segments the filling and not the entire tooth. We believe that this issue could be solved by having a annotation label that indicate the presence of amalgam filling for each tooth. That way, the model could be trained to detect these fillings and overcome this issue.

% At last, we want to propose some ideas of research in this field that can be studied in order to solve interesting problems. Our initial plan in this work was to use annotations made by professional dentists, those would include different classes for each tooth and many health properties of each tooth. Having such annotations, one can train a model that can predict each type of tooth separately, meaning that instead of predicting all Gaussians in one heatmap, the model would predict one heatmap for each tooth. This would also open more possibilities for instance segmentation. Also, if the model would have been trained to classify images based on the tooth diseases, it perhaps could be further expanded to detecting these diseases in the input image. Also, the transformer architectures are getting more and more popular for image processing, because of the attention mechanism. It is a powerful mechanism that enables the model to learn features more effectively and can also be exploited in the weakly supervised or unsupervised training. One idea for improvement could be for example to train vision transformer in self-supervised manner (as described in \cite{cutler}) on our dataset. Therefore, our future work in this field would certainly include the usage of vision transformers.





==> tables/a-thresh-results.tex <==
\begin{table}[b!]
\centering
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
  Image type & Metric & Lower jaw only & Front view only & Upper jaw only  \\
 \hline
 \multirow{4}{*}{Original} 
& IoU & \textbf{0.501} & 0.085 & \textbf{0.382}  \\ 
& Precision & \textbf{0.528} & 0.281 & \textbf{0.397}  \\ 
& Recall & 0.818 & 0.137 & 0.789 \\ 
& F1 score &\textbf{0.642} & 0.185 & 0.528 \\ 
 \hline
 \multirow{4}{*}{Inpainted} 
& IoU & 0.496 & \textbf{0.278} & 0.377  \\ 
& Precision & 0.508 & \textbf{0.469} & 0.376  \\ 
& Recall & \textbf{0.858} & \textbf{0.559} & \textbf{0.799} \\ 
& F1 score & 0.638 & \textbf{0.51} & 0.511 \\ 
 \hline
\end{tabular}
\caption{Automatic thresholding segmentation results. Everything was evaluated on the image size of 512x512 pixels. Bold values represent the best value of a metric for a certain dataset.}
\label{table:a-thresh-results}
\end{table}

==> tables/cutler-results.tex <==
\begin{table}[b!]
\centering
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
  Image type & Metric & Lower jaw only & Front view only & Upper jaw only  \\
 \hline
 \multirow{4}{*}{Original} 
& IoU & \textbf{0.413} & 0.307 & \textbf{0.269} \\
 & Precision & \textbf{0.4} & 0.317 & \textbf{0.272} \\
 & Recall & \textbf{0.746} & \textbf{0.724} & \textbf{0.762} \\
 & F1 score & \textbf{0.52} & 0.441 & \textbf{0.401} \\
\hline
\multirow{4}{*}{Inpainted}
& IoU & 0.32 & \textbf{0.316} & 0.24 \\
 & Precision & 0.345 & \textbf{0.331} & 0.244 \\
 & Recall & \textbf{0.746} & 0.719 & 0.684 \\
 & F1 score & 0.472 & \textbf{0.454} & 0.359 \\
 \hline
\end{tabular}
\caption{CutLER segmentation results. Everything was evaluated on the image size of 512x512 pixels. Bold values represent the best value of a metric for a certain dataset.}
\label{table:cutler-results}
\end{table}

==> tables/feature-map-thresholding.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison of results from thresholding. Bold values represent the best value of a metric for a certain dataset.}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
  Image type & Metric & Lower jaw only & Front view only & Upper jaw only  \\
 \hline
\multirow{4}{*}{Original images}
& IoU & 0.537 & 0.57 & 0.427 \\
 & Precision & 0.536 & 0.638 & 0.419 \\
 & Recall & \textbf{0.897} & 0.824 & \textbf{0.864} \\
 & F1 score & 0.671 & 0.719 & 0.565 \\
\hline
\multirow{4}{*}{Feature maps} 
& IoU & \textbf{0.619} & \textbf{0.635} & \textbf{0.487} \\
 & Precision & \textbf{0.686} & \textbf{0.673} & \textbf{0.478} \\
 & Recall & 0.863 & \textbf{0.927} & 0.768 \\
 & F1 score & \textbf{0.764} & \textbf{0.78} & \textbf{0.589} \\
 \hline
\end{tabular}
\label{table:thresholding-comparison}
\end{table*}

==> tables/hsv-masks.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{ |m{3cm}|M{3cm}|M{3cm}| } 
 \hline
  & First mask & Second mask  \\
 \hline
 Lower bound & [0, 50, 50] & [170, 50, 50] \\ 
 \hline
 Upper bound & [4, 255, 255] & [180, 255, 255] \\ 
 \hline
\end{tabular}
\caption{Lower and upper bounds for two masks used in thresholding HSV color space. The numbers in the lists correspond to hue, saturation and value.}
\label{table:hsv-masks}
\end{table}

==> tables/hsv-thresh-results.tex <==
\begin{table}[b!]
\centering
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
  Image type & Metric & Lower jaw only & Front view only & Upper jaw only  \\
 \hline
 \multirow{4}{*}{Original} 
& IoU & \textbf{0.601} & \textbf{0.581} & 0.441 \\
 & Precision & 0.574 & \textbf{0.591} & 0.408 \\
 & Recall & \textbf{0.982} & \textbf{0.965} & \textbf{0.992} \\
 & F1 score & 0.724 & \textbf{0.733} & \textbf{0.578} \\
\hline
\multirow{4}{*}{Inpainted}
& IoU & \textbf{0.601} & 0.553 & \textbf{0.443} \\
 & Precision & \textbf{0.582} & 0.588 & \textbf{0.41} \\
 & Recall & 0.959 & 0.911 & 0.979 \\
 & F1 score & \textbf{0.725} & 0.714 & \textbf{0.578} \\
 \hline
\end{tabular}
\caption{HSV thresholding segmentation results. Everything was evaluated on the image size of 512x512 pixels. Bold values represent the best value of a metric for a certain dataset.}
\label{table:hsv-thresh-results}
\end{table}

==> tables/keypoint-results-all-images.tex <==
\begin{table}[htbp]
\caption{Keypoint prediction results on dataset containing all images from the dataset. Every metric was evaluated with respect to input resolution of 512x512 pixels. Each value (mean, median) is calculated in image pixels.}
\centering
\begin{tabular}{|c|c|c|} 
 \hline
  \textbf{Output resolution (px)} & \textbf{Metric} & \textbf{All images}  \\
 \hline
\multirow{2}{*}{128x128} 
& mean (px) & \textbf{9.07} \\ 
& median (px) & \textbf{6.43}\\ 
\hline
\multirow{2}{*}{512x512}
& mean (px)& 13.92 \\ 
& median (px)& 6.7  \\ 
 \hline
\end{tabular}

\label{table:keypoint-results-all-images}
\end{table}

==> tables/keypoint-results-augment.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{ |c|c|p{1.5cm}|p{1cm}|p{1cm}|p{1cm}|p{2cm}| } 
 \hline
  Augmentation & Metric & All images & Lower jaw only & Front view only & Upper jaw only & Lower and upper jaw only  \\
 \hline
\multirow{ 2}{*}{None} 
& mean (px)  & 13.92 & 7.39 & 13.65 & 6.97 & 7.29 \\ 
& median (px) & \textbf{6.7} & \textbf{5.68} & \textbf{5.7} & 6.14 & 5.52 \\ 
\hline
\multirow{ 2}{*}{Flip}
& mean (px) & \textbf{12.69} & \textbf{7.37} & \textbf{9.12} & 6.39 & 6.75 \\ 
& median (px)& 7.07 & 5.98 & 6.08 & 5.5 & 5.71 \\ 
\hline
\multirow{ 2}{*}{Rotate}
& mean (px) & 14.55 & 9.95 & 14.07 & 7.98 & 8.52 \\ 
& median (px)& 7.28 & 7.04 & 6.63 & 6.5 & 6.36 \\ 
\hline
\multirow{ 2}{*}{Translate}
& mean (px) & 12.97 & 9.2 & 10.98 & 6.44 & 7.11 \\ 
& median (px)& 6.74 & 5.94 & 6.0 & 5.68 & 6.36 \\ 
\hline
\multirow{ 2}{*}{F+R+T}
& mean (px) & 17.24 & 11.61 & 14.36 & 7.94 & 7.68 \\ 
& median (px)& 7.14 & 6.51 & 6.71 & 6.4 & 6.04 \\ 
\hline
\multirow{ 2}{*}{Brightness}
& mean (px) & 16.54 & 7.41 & 9.21 & 6.66 & \textbf{6.72} \\ 
& median (px)& 7.07 & 5.89 & 6.08 & 5.86 & 5.55 \\ 
\hline
\multirow{ 2}{*}{Contrast}
& mean (px) & 21.34 & 7.61 & 26.15 & \textbf{6.3} & 6.82 \\ 
& median (px)& 7.21 & 6.36 & 7.07 & \textbf{5.49} & 5.66 \\ 
 \hline
\end{tabular}
\caption{Keypoint prediction results with data augmentation. Left-most column shows the augmentation type, F+R+T is flip, rotate and translate together. Everything was evaluated with respect to input resolution of 512x512 pixels. Each value (mean, median) is calculated in image pixels.}
\label{table:keypoint-results-augment}
\end{table}

==> tables/keypoint-results-backbones.tex <==
\begin{table}[b!]
\centering
\begin{tabular}{ |c|p{2.4cm}|c|p{2cm}|p{2cm}|p{2.7cm}| } 
 \hline
  Backbone & Output resolution (px) & Metric & All images & Front view only & Lower and upper jaw only  \\
 \hline
 \multirow{4}{*}{ResNet50} & \multirow{ 2}{*}{128x128} 
& mean (px)  & 9.71 & 11.11 & 8.49  \\ 
& & median (px) & 7.81 & 7.63 & 7.65  \\ 
\cline{2-6}
& \multirow{ 2}{*}{512x512}
& mean (px) & \textbf{7.63} & 10.15 & 7.46 \\ 
& & median (px)& 6.0 & 6.36 & 6.28 \\ 
 \hline
 \multirow{4}{*}{Hourglass} & \multirow{ 2}{*}{128x128} 
& mean (px)  & 8.88 & 13.51 & 8.06  \\ 
& & median (px) & 7.07 & 8.25 & 6.3  \\ 
\cline{2-6}
& \multirow{ 2}{*}{512x512} 
& mean (px) & 8.14 & \textbf{9.41} & \textbf{7.26} \\ 
& & median (px)& \textbf{5.67} & \textbf{5.83} & \textbf{5.05} \\ 
 \hline
\end{tabular}
\caption{Keypoint prediction results. Everything was evaluated with respect to input resolution of 512x512 pixels. Each value (mean, median) is calculated in image pixels.}
\label{table:keypoint-results-backbones}
\end{table}

==> tables/keypoint-results-basic.tex <==
\begin{table*}[t!]
\centering
\caption{Keypoint prediction results. Everything was evaluated with respect to input resolution of 512x512 pixels. Each value (mean, median) is calculated in image pixels.}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
  Output resolution (px) & Metric & All images & Lower jaw only & Front view only & Upper jaw only & Lower and upper jaw only  \\
 \hline
\multirow{ 2}{*}{128x128} 
& mean (px) & 9.07 & 14.86 & 16.17 & \textbf{6.82} & 8.83 \\ 
& median (px) & 6.43 & 8.5 & 12.31 & 6.45 & 7.93 \\ 
\hline
\multirow{ 2}{*}{512x512}
& mean (px) & 13.92 & \textbf{7.39} & \textbf{13.65} & 6.97 & \textbf{7.29} \\ 
& median (px) & 6.7 & \textbf{5.68} & \textbf{5.7} & \textbf{6.14} & \textbf{5.52} \\ 
 \hline
\end{tabular}
\label{table:keypoint-results-basic}
\end{table*}

==> tables/our-results.tex <==
\begin{table}[b!]
\centering
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
  Image type & Metric & Lower jaw only & Front view only & Upper jaw only  \\
 \hline
 \multirow{4}{*}{Original} 
& IoU & \textbf{0.876}& \textbf{0.775} & 0.669 \\
 & Precision & 0.955 &\textbf{0.801} & 0.891 \\
 & Recall & \textbf{0.914} & \textbf{0.952} & 0.731 \\
 & F1 score & \textbf{0.934} & \textbf{0.87} & 0.803 \\
\hline
\multirow{4}{*}{Inpainted}
& IoU & 0.846 & 0.717 & \textbf{0.74} \\
 & Precision & \textbf{0.96} & 0.774 & \textbf{0.893} \\
 & Recall & 0.872 & 0.899 & \textbf{0.806} \\
 & F1 score & 0.914 & 0.832 & \textbf{0.847} \\
 \hline
\end{tabular}
\caption{Results from our proposed method. Everything was evaluated on the image size of 512x512 pixels. Bold values represent the best value of a metric for a certain dataset.}
\label{table:our-results}
\end{table}

==> tables/sam-results.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
  Mode & Image type & Metric & Lower jaw only & Front view only & Upper jaw only  \\
 \hline
 \multirow{8}{*}{Auto} & \multirow{4}{*}{Original} 
& IoU & 0.369 & 0.377 & 0.367 \\
 & & Precision & 0.336 & 0.35 & 0.339 \\
 & & Recall & \textbf{0.963} & \textbf{0.95} & \textbf{0.973} \\
 & & F1 score & 0.498 & 0.512 & 0.502 \\
\cline{2-6}
& \multirow{4}{*}{Inpainted}
& IoU & 0.317 & 0.311 & 0.358 \\
 & & Precision & 0.317 & 0.315 & 0.35 \\
 & & Recall & 0.901 & 0.812 & 0.888 \\
 & & F1 score & 0.469 & 0.454 & 0.502 \\
 \hline
\multirow{8}{*}{Keypoints} & \multirow{4}{*}{Original} 
& IoU & \textbf{0.876} & \textbf{0.555} & \textbf{0.909} \\
 & & Precision & \textbf{0.922} & \textbf{0.526} & \textbf{0.975} \\
 & & Recall & 0.943 & 0.944 & 0.928 \\
 & & F1 score &\textbf{0.932} & \textbf{0.675} & \textbf{0.951} \\
\cline{2-6}
& \multirow{4}{*}{Inpainted}
& IoU & 0.83 & 0.477 & 0.799 \\
 & & Precision & 0.907 & 0.442 & 0.826 \\
 & & Recall & 0.895 & 0.958 & 0.877 \\
 & & F1 score & 0.901 & 0.605 & 0.85 \\
 \hline
\end{tabular}
\caption{Results using Segment Anything Model. Everything was evaluated on the image size of 512x512 pixels. First half of table contains results obtained using the automatic mode, second half is obtained by using predicted keypoints as reference points. Bold values represent the best value of a metric for a certain dataset.}
\label{table:sam-results}
\end{table*}

==> tables/summary-results.tex <==
\begin{table*}[t!]
\centering
\caption{Summary results from every method on complete dataset of all images. Everything was evaluated on the image size of 512x512 pixels. Bold values represent the best values of each metric.}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
   Metric & Automatic thresholding & HSV thresholding & Our method & SAM auto & SAM per point \\
 \hline
 IoU & 0.323 & 0.541 & \textbf{0.785} & 0.371 & 0.737\\
 Precision & 0.432 & 0.514 & \textbf{0.86} & 0.342 & 0.71 \\
 Recall & 0.558 & \textbf{0.979} & 0.891 & 0.961 & 0.839 \\
 F1 score & 0.487 & 0.674 & \textbf{0.875} & 0.504  & 0.769 \\
\hline
\end{tabular}
\label{table:summary-results}
\end{table*}
